Private Electronic Payments with Self-Custody and Zero-Knowledge Verified Reissuance

This article builds upon the protocol for digital transfers described by Goodell, Toliver, and Nakib, which combines privacy by design for consumers with strong compliance enforcement for recipients of payments and self-validating assets that carry their own verifiable provenance information. We extend the protocol to allow for the verification that reissued assets were created in accordance with rules prohibiting the creation of new assets by anyone but the issuer, without exposing information about the circumstances in which the assets were created that could be used to identify the payer. The modified protocol combines an audit log with zero-knowledge proofs, so that a consumer spending an asset can demonstrate that there exists a valid entry on the audit log that is associated with the asset, without specifying which entry it is. This property is important as a means to allow money to be reissued within the system without the involvement of system operators within the zone of control of the original issuer. Additionally, we identify a key property of privacy-respecting electronic payments, wherein the payer is not required to retain secrets arising from one transaction until the following transaction, and argue that this property is essential to framing security requirements for storage of digital assets and the risk of blackmail or coercion as a way to exfiltrate information about payment history. We claim that the design of our protocol strongly protects the anonymity of payers with respect to their payment transactions, while preventing the creation of assets by any party other than the original issuer without destroying assets of equal value.

==> UC.tex <==
\subsection{Universal Composability}

In the UC model~\cite{Canetti01} we distinguish between ideal and real execution.

\paragraph{The Real Execution.}
In the real world, the protocol $\pi$ is run in the presence of an adversary $\advA$ coordinated by a non-uniform environment $\advZ = \{\advZ_\secpar\}_{\secpar\in\NN}$.
At the outset, $\advZ$ chooses the inputs $(1^\secpar,\inp_i)$ for each player $\party_i$, and gives $\calI$, $\{\inp_i\}_{i\in\calI}$ and $z$ to $\advA$, where $\calI \subset [\num]$ represents the set of corrupted players and $z$ is some auxiliary input. For simplicity, we only consider static corruptions (i.e.,\ the environment decides who is corrupt at the beginning of the protocol).
The parties then start running $\pi$, with the honest players $\party_i$ behaving as prescribed in the protocol (using input $x_i$), and with malicious parties behaving arbitrarily (directed by $\advA$). The attacker may delay sending the messages of the corrupted parties in any given phase until after the honest parties send their messages in that phase. $\advZ$ can interact with $\advA$ throughout the course of the protocol execution.

 Additionally, $\advZ$ receives the outputs of the honest parties, and must output a bit. We denote by $\REAL_{\pi,\advA,\advZ}(\secpar)$ the random variable corresponding to $\advZ$'s guess.

\paragraph{The Ideal Execution.}
In the ideal world, a trusted third party evaluates the functionality $\Func$ on behalf of a set of dummy players $(\party_i)_{i \in [\num]}$. As in the real setting, $\advZ$ chooses the inputs $(1^\secpar,\inp_i)$ for each honest player $\party_i$, and gives $\calI$, $\{\inp_i\}_{i\in\calI}$ and $z$ to the ideal adversary $\advS$, corrupting the dummy parties $(\party_i)_{i \in \calI}$. Hence, honest parties send their input $x_i' = x_i$ to the trusted party, whereas the parties controlled by $\advS$ might send an arbitrary input $x_i'$. The trusted party computes behaves as prescribed by $\Func$.
During the simulation, $\advS$ can interact with $\advZ$ throughout the course of the protocol execution.
 Additionally, $\advZ$ receives the outputs of the honest parties and must output a bit. We denote by $\IDEAL_{\Func,\advS,\advZ}(\secpar)$ the random variable corresponding to $\advZ$'s guess.

\begin{definition}[UC-Secure MPC]\label{def:mpc}
Let $\pi$ be an $\num$-party protocol for computing a functionality $\Func$. We say that $\pi$ $\thr$-realizes $\Func$ in the presence of malicious adversaries if  for every PPT adversary $\advA$ there exists a PPT simulator $\advS$ such that for every non-uniform PPT environment $\advZ$ corrupting at most $t$ parties it holds that
$$
\Big\{\REAL_{\pi,\advA,\advZ}(\secpar)\Big\}_{\secpar\in\NN} \cind \Big\{\IDEAL_{\Func,\advS,\advZ}(\secpar)\Big\}_{\secpar\in\NN}.
$$
%When replacing $\IDEAL_{\Func,\advS,\advZ}(\secpar)$ with $\IDEAL_{\Func_\bot,\advS,\advZ}(\secpar)$ we say that $\pi$ $\thr$-securely computes $\Func$ {\em with aborts} in the presence of malicious adversaries.


\end{definition}

%Hence, we also consider a weakening of the ideal process involving a functionality $\Func_{\func}^\bot$ which behaves identically to $\Func_\func$ except that:
%(i) When the trusted party computes the outputs $(\out_1,\ldots,\out_n)$, it first gives $(\out_i)_{i\in\calI}$ of the corrupted players 
%to the simulator; and
%(ii) The simulator may send either a message $\mathtt{continue}$ or $\mathtt{abort}$ to the trusted party: in the former case, the trusted party sends the 
%output $\out_i$ to all honest players, in the latter case they
%receive an abort symbol $\bot$. All of the provably secure constructions that we will present we assume that the adversaries are static, i.e. that are fixed at the beginning of the execution.
\ignore{
\paragraph{Generalized UC.} An even stronger composability guarantee is that of \emph{generalized} UC~\cite{CanettiDPW07}. Roughly, in this setting, entities have black-box access to one or more global functionalities. A global functionality is an external functionality accessible by both the real and ideal world entities. The same instance of a global functionality can be accessed by multiple protocols (either simultaneously or sequentially depending on the model).

\begin{definition}[GUC-Secure MPC]\label{def:mpc}
Let $n\in\NN$.
Let $\Func_f,\GFunc_g$ be ideal functionalities for $\func,\gunc:
(\bin^*)^n \rightarrow (\bin^*)^n$, and let $\pi$ be an $n$-party protocol.
We say that $\pi_f$ $t$-securely realizes in the $\GFunc_g$-GUC model if in the presence of malicious adversaries if  for every PPT adversary $\advA$ there exists a PPT simulator $\advS$ such that for every non-uniform PPT environment $\advZ$ corrupting at most $t$ parties the following holds:
\[
\left\{\REAL^g_{\pi,\advA,\advZ}(\secpar)\right\}_{\secpar\in\NN} \cind \left\{\IDEAL^g_{\func,\advS,\advZ}(\secpar)\right\}_{\secpar\in\NN}.
\]
where $g$ on top of the experiments $\REAL$ and $\IDEAL$ means that both experiments have black-box access to the function $g$.
\end{definition}
\paragraph*{The MPC Hybrid Model.}
Let $\HYBRID^{\GFunc_1,\ldots,\GFunc_\tau}_{\pi,\advA,\advZ}(\secpar)$ denote the random variable 
corresponding to the output of $\advZ$ in the $(\GFunc_1,\ldots,\GFunc_\tau)$-hybrid model.
We say that a protocol $\pi$ for computing $\Func$ is secure in the $(\GFunc_1,\ldots,\GFunc_\tau)$-hybrid model if the ensembles $\HYBRID^{(\GFunc_1,\ldots,\GFunc_\tau)}_{\pi,\advA,\advZ}(\secpar)$ and $
\IDEAL_{\Func,\Sim,\advZ}(\secpar)$ are computationally close.
}
\begin{definition}[UC-Secure MPC in the hybrid model]\label{def:uc-hybrid}
	Let $n\in\NN$.
	Let $\Func$ and $\GFunc_1,\ldots,\GFunc_\tau$ be ideal functionalities,
 and let $\pi$ be an $n$-party protocol.
	We say that $\pi$ $\thr$-securely realizes $\Func$ in the $(\GFunc_1,\ldots,\GFunc_\tau)$-
hybrid model if for all PPT adversaries $\advA$ there exists a PPT simulator $\Sim$ 
such that for all PPT non-uniform environments $\advZ$ corrupting at most $\thr$ 
players, then
	$$
	\Big\{\IDEAL_{\Func,\Sim,\advZ}(\secpar)\Big\}_{\secpar\in\NN} 
	\cind 
	\left\{\HYBRID^{\GFunc_1,\ldots,\GFunc_\tau}_{\pi,\advA,\advZ}(\secpar)\right\}_{\secpar\in\NN}.
$$
\end{definition}
%The same definitions are applicable to the stand-alone setting by replacing the environment with a distinguisher $\advD$. He can only handle inputs to the parties and receive back an arbitrary function of $\advA$'s view, and then outputs a bit.
\ignore{
We further introduce the GUC variant of the MPC hybrid model.
\begin{definition}[GUC-Secure MPC in the hybrid model]\label{def:uc-hybrid}
	Let $n\in\NN$.
	Let $\Func_\func$, $\Func_\gunc$, and $\GFunc_h$ be ideal functionalities for $\func,\gunc,h:
(\bin^*)^n \rightarrow (\bin^*)^n$, and let $\pi$ be an $n$-party protocol.
	We say that $\pi$ $\thr$-securely realizes $\Func_\func$ in the $\Func_\gunc$-
hybrid $\GFunc_h$-GUC model if for all PPT adversaries $\advA$ there exists a PPT simulator $\Sim$ 
such that for all PPT non-uniform environments $\advZ$ corrupting at most $\thr$ 
players, we have
	\begin{equation*}
	\left\{\IDEAL^h_{\func,\Sim,\advZ}(\secpar)\right\}_{\secpar\in\NN} 
	\cind 
	\left\{\HYBRID^{\gunc,h}_{\pi,\advA,\advZ}(\secpar)\right\}_{\secpar\in\NN}.
	\end{equation*}	
\end{definition}
}

\paragraph{Disjoint Parties Variant.}
In our setting, we are considering a slightly different corruption model taking into account multiple set of parties, in which the adversary have the power to corrupt at most a certain number of parties for each set.
   We call a protocol with involved parties $\parties=(\parties_1,\ldots,\parties_m)$ where $|\parties_i|=n_i$ for $i\in[m]$ an $(n_1,\ldots,n_m)$-party protocol.


\begin{definition}[Disjoint Parties UC-Secure MPC in the Hybrid Model]\label{def:mult-parties-uc}
	Let $m\in\NN$ and $n_i\in\NN$ for $i\in[m]$. Let $\parties=(\parties_1,\ldots,\parties_m)$ where $|\parties_i|=n_i$ for $i\in[m]$.
	Let $\Func$ and $\GFunc_1,\ldots,\GFunc_\tau$, be ideal functionalities and let $\pi$ be an $(n_1,\ldots,n_m)$-party protocol.
	We say that $\pi$ $(\thr_1,\ldots,\thr_m)$-securely realizes $\Func$ in the $(\GFunc_1,\ldots,\GFunc_\tau)$-hybrid model if for all PPT adversaries $\advA$ there exists a PPT simulator $\Sim$ 
such that for all PPT non-uniform environments $\advZ$ corrupting at most $\thr_i$ players in $\parties_i$ for $i\in[m]$, then
$$
	\Big\{\IDEAL_{\Func,\Sim,\advZ}(\secpar)\Big\}_{\secpar\in\NN} 
	\cind 
	\left\{\HYBRID^{\GFunc_1,\ldots,\GFunc_\tau}_{\pi,\advA,\advZ}(\secpar)\right\}_{\secpar\in\NN}.
$$
\end{definition}
\ignore{
\begin{definition}[Disjoint Parties GUC-Secure MPC in the Hybrid Model]\label{def:mult-parties-guc}
	Let $m\in\NN$ and $n_i\in\NN$ for $i\in[m]$. Let $\parties=(\parties_1,\ldots,\parties_m)$ where $|\parties_i|=n_i$ for $i\in[m]$.
	Let $\Func_\func$, $\Func_\gunc$, and $\GFunc_h$ be ideal functionalities for $\func,\gunc,h:
(\bin^*)^{\sum_{i\in[m]}n_i} \rightarrow (\bin^*)^{\sum_{i\in[m]}n_i}$, and let $\pi$ be an $(n_1,\ldots,n_m)$-party protocol.
	We say that $\pi$ $(\thr_1,\ldots,\thr_m)$-securely realizes $\Func_\func$ in the $\Func_\gunc$-
hybrid $\GFunc_h$-GUC model if for all PPT adversaries $\advA$ there exists a PPT simulator $\Sim$ 
such that for all PPT non-uniform environments $\advZ$ corrupting at most $\thr_i$ players in $\parties_i$ for $i\in[m]$, we have
	\begin{equation*}
	\left\{\IDEAL^h_{\func,\Sim,\advZ}(\secpar)\right\}_{\secpar\in\NN} 
	\cind 
	\left\{\HYBRID^{\gunc,h}_{\pi,\advA,\advZ}(\secpar)\right\}_{\secpar\in\NN}.
	\end{equation*}	
\end{definition}
}

==> bibliography.tex <==
\bibitem{goodell2022}{
    G Goodell, D Toliver, and H Nakib.
    ``A Scalable Architecture for Electronic Payments.''
    In: S Matsuo et al., \textit{Financial Cryptography and Data Security}.
    FC 2022 International Workshops. FC 2022.
    \textit{Lecture Notes in Computer Science} 13412,
    2023.
    Springer, Cham.
    [online]
    \url{https://doi.org/10.1007/978-3-031-32415-4_38}
}
\bibitem{chaum1982}{
    D. Chaum.
    ``Blind Signatures for Untraceable Payments.''
    \textit{Advances in Cryptology: Proceedings of Crypto}
    \textbf{82}(3), 
    pp. 199--203,·
    1983.
    [online]
    \url{http://www.hit.bme.hu/~buttyan/courses/BMEVIHIM219/2009/Chaum.BlindSigForPayment.1982.PDF}
    [retrieved 2018-09-28]
}





==> ledgerprot.tex <==
\begin{figure}[t]
\begin{framed}
    $\smc$ interacts with the other parties as follows, depending on the protocol running phase.
\begin{description}
\item[Setup:] During the setup phase, first instantiate a set of minters' verification keys $\mintkeys=\emptyset$ and empty set of assets $\assetvar=\emptyset$, and then
\begin{itemize}
    \item Upon receiving the central bank verification key $\vk^{\cbank}$ from $\cbank$, store it and broadcast it to all the parties. Any other message from $\cbank$ is then discarded.
    \item Upon receiving $(\SET,\{\vk_\minter\},\vkfrom,\vkto,\sigma^{\cbank})$ from the central bank $\cbank$, check that $\BS.\ver(\vk^{\cbank},(\crs,\{\vk_\minter\},\{(\vkfrom,\vkto)\}),\sigma^{\cbank})=1$. If the check passes, set $\mintkeys = \{\vk_\minter\}$ and $\assetvar=\{(\vkfrom,\vkto,0)\}$. Broadcast $\mintkeys$ and $\assetvar$ to all the parties.
\end{itemize}
 

    \item[Asset update:] Upon receiving $(\UPDATE,\vkfrom,\vkto,\sigmafrom,\vk_T,\sigma_T,\pi)$ in from any party  $\party\in\parties$, checks that:
        \begin{itemize}
        \item $\vk_T \in \mintkeys$
         \item $(\vkfrom,\cdot,\cdot)\notin\assetvar$.
             \item $\BS.\ver(\vk^\minter,\vkfrom,\sigma_\minter)=1$.
             \item  $\BS.\ver(\vkfrom,(\vkfrom,\vkto),\sigmafrom)=1$ (i.e. the sender certifies knowledge of the signing key relative to $\vkfrom$).
             \item $\nizk.\ver(\crs,(\beta_1,\ldots,\beta_n,\vk^\sender),\pi)=1$, where $\blinded_1,\ldots,\blinded_n$ are the blinded generation assets related to burnt assets.
    \end{itemize}
    If all the checks pass, add $(\vkfrom,\vkto,0)$ to $\assetvar$ and broadcast $(\UPDATED,\vkfrom,\vkto)$ to all the parties.

\item[Asset burn:] Upon receiving $(\SPEND,\vkfrom,\vkto,\sigma_T,\sigmato,\vk^\minter,\blinded)$ from a party $\party\in\parties$, checks that:
\begin{itemize}
        \item $\vk_T \in \mintkeys$.
    \item $\BS.\ver(\vk^T,(\vkfrom,\vkto,\sigmato),\sigma_T)=1$.
    \item $(\vkfrom,\vkto,1)\notin\assetvar$ (i.e., the asset was not burned previously).
    \item $\BS.\ver(\vkto,(\vkfrom,\vkto),\sigmato)=1$ (i.e., $\vkto$ is the recipient of the asset).

\end{itemize}
If the checks above pass add $(\vkfrom,\vkto,\blinded)$ to $\assetvar$ and broadcast $(\SPENT,\vkfrom,\vkto)$ to all the parties.
\end{description}
    
\end{framed}
    \caption{Smart Contract $\smc$}
    \label{fig:funcsc}
\end{figure}
Further, the protocol is instantiated with a function $\checkreg(\cdot)$ run by the banks to check for regulation compliance.

 \begin{figure}[t]
     \begin{framed}

\begin{center}
    \textbf{Protocol} $\pidc^\tau$
\end{center}
    %\footnotesize
The protocol is divided into the following phases:
\begin{description}
\item[Asset distribution:] 
Parties behave as follows:

%(we assume that they all requested the same amount for the aim of simplicity).
%The central bank $\cbank$, owning a certified verification key $\vk^{\cbank}$ and the corresponding signing key $\sk^{\cbank}$.

%proceeds as follows:

\begin{itemize}
    \item All the parties wait to receive the central bank verification key $\vkcb$ from $\cbank$.
    \item Each minter $\minter\in\minters$ computes $(\vk^\minter,\sk^\minter)\getsr\Gen(1^\secpar)$ and sends $\vk^\minter$ to $\cbank$.
  
\end{itemize}

    \item[Asset creation:] 
    $\sender$, owning an asset $F_1=(\vk,\vk')$ intaract with their bank $\bank$ as follows:
    \begin{itemize}
        \item $\sender$ computes $(\vk^\sender,\sk^\sender)\getsr\BS.\Gen(1^\secpar)$ and $(\blinded^\sender,\bfactor^\sender)=\blind(\vk^S;r)$ for a random $r\gets\bin^\secpar$.
        Then, computes $\sigma'\getsr\BS.\sign(\sk',F_1)$
      and sends $(F_1,\sigma')$ together with the blinded message $\blinded^\sender$ to $\bank$. $\bank$ will, in turn, forward $(F_1,\sigma',\blinded^\sender)$ to his own minter $\minter_\bank\in\minters$.
        \item $\minter_\bank$ computes a signature $\sigma_\minter\getsr\BS.\sign(\sk^\minter,(F_1,\sigma'))$ and
       sends $(\SPEND,F_1,\sigma',\vk^\minter,\sigma_\minter,\blinded^\sender)$ to $\smc$.
        If receiving $(\SPENT,F_1)$ from $\smc$, $\minter$
        generates $\bsigma^{\minter_\bank}\getsr\BS.\bsign(\sk^{\minter_\bank},\blinded^\sender)$ and forwards $\bsigma^{\minter_\bank}$ to $\bank$, that, in turn, forwards $\bsigma^{\minter_\bank}$ to $\sender$.
        \item $\sender$ can now obtain a signature $\sigma^{\minter_\bank}=\unblind(\bsigma^{\minter_\bank},\bfactor^\sender)$. Hence, $\sender$ can now construct an asset $F_0^\sender=(\vk^\sender,\sigma^{\minter_\bank})$. %and queries $\FuncVer$ with $(\CREATE,\vk^{\sender},\sigma^{\minter_\bank})$.
    \end{itemize}
 \item[Asset transfer:] 
 $\sender$ owns an asset $F_0^\sender=(\vk^\sender,\sigma^{\minter_\bank})$ such that $\BS.\ver(\vk^{\minter_\bank},F_0^\sender)=1$.
 The sender $\sender$, the receiver $\receiver$, and the receiver's bank $\bank^\receiver$, interact as follows:
 \begin{itemize}
    \item $\receiver$ computes $(\vk^\receiver,\sk^\receiver)\getsr\BS.\Gen(1^\secpar)$ and sends $\vk^\receiver$ to $\sender$.
     \item $\sender$
     generates a signature $\sigma^\sender\getsr\sign(\allowbreak\sk^\sender,\allowbreak (F_1^{(\sender,\receiver)}=(\vk^\sender,\vk^\receiver),\sigma^{\minter_\bank}))$. Let  $(\blinded_1,\ldots,\blinded_n)$ be the list of the blinded messages related to the burnt tokens, $i$ such that $\blinded_i=\blinded^\sender$. Then, 
 computes $\pi\getsr\nizk.\prove(\crs,(\beta_1,\ldots,\beta_n,\vk^\sender),(r,i))$
     and sends $(F_1^{(\sender,\receiver)},\sigma^\sender,\pi)$ to $\receiver$.
     \item $\receiver$, now owning an updated asset $F_1^{(\sender,\receiver)}=(\vk^\sender,\vk^\receiver)$ together with the minter signature $\sigma^{\minter_\bank}$, generates a signature $\sigma^\receiver\getsr\BS.\sign(\sk^\receiver,(F_1^{(\sender,\receiver)},\sigma^{\minter_\bank}))$ and sends $(F_1^{(\sender,\receiver)},\sigma^{\minter_\bank},\sigma^\sender,\sigma^\receiver,\pi)$ to his own bank $\bank'$.
     \item $\bank'$ checks if $\checkreg(F_1^{(\sender,\receiver)},\sigma^{\minter_\bank},\sigma^\sender,\sigma^\receiver,\assetvar)=0$ (i.e., the asset is not regulation compliant). If so, denies the receiver's payment and aborts the execution. Else, queries $\FuncSC$ with $(\UPDATE,F_1^{(\sender,\receiver)},\sigma^{\minter_\bank},\sigma^\sender,\vk^{\minter_\bank},\pi)$. 
     \item $\receiver$, when receiving  $(\UPDATED,\vk^\sender,\vk^\receiver)$ from $\FuncSC$ accepts the receiver's payment. Otherwise, denies the receiver's payment.
    
 \end{itemize}

 
  
\end{description}

     \end{framed}
     \caption{Our protocol $\pidc$.}
     \label{fig:pidc}
 \end{figure}



==> ourprotocol.tex <==
Let us consider the following functionality:

\begin{framed}
    \begin{center}
       {\bf Functionality $\FuncVer$} 
    \end{center}
    The functionality runs with a set of users $\users$, banks $\banks$, minters $\minters$, central bank $\cbank$, a blind signature scheme $\BS=(\BS.\Gen,\BS.\sign,\BS.\bsign,\BS.\blind,\BS.\unblind,\BS.\ver)$, a central bank's verification key $\vk^{\cbank}$, a set of genesis assets $\{\vk_i\}_{i\in[\genassets]}$, a set of $|\minters|$ verification keys $\{\vk^\minter\}_{\minter\in\minters}$. It is also initialized with a vector $\assetvar$, where $\assetvar[i]=(\vk^{\cbank},\vk_i,0)$ for each $i\in[\genassets]$. Each of the entries of $\assetvar$ will be append-only. 
    %From now on, we will refer as $\genassets_i$ as the actual size of the $i$-th vector in the matrix.
    The functionality is further initialized with an auxiliary function $f_\aux(\assetvar)$, that will be used by the banks to guarantee regulations. 
    It is divided in the following phases:
\begin{description}
  %  \item[Asset creation:] Upon receiving $(\CREATE,\vkfrom,\sigma^\minter)$ from a user $\user\in\users$:
 %   \begin{itemize}
  %       \item For each $i\in[\genassets]$,  check that
 %     $\assetvar[i]\ne(\vkfrom,\cdot)$ (i.e. $\vkfrom$ is fresh).
   %           \item Check that $\BS.\ver(\vk^\minter,\vkfrom,\sigma_\minter)=1$.

 %   \end{itemize}
 %   If all the checks pass, set $\assetvar[\genassets+1]=(\vkfrom,\bot)$.

    \item[Asset update:] Upon receiving $(\UPDATE,\vkfrom,\vkto,\sigmafrom)$ from a party  $\party\in\banks\cup\users$, does as follows:
    \begin{itemize}
         \item For each $i\in[\genassets]$,  check that
      $\assetvar[i]\ne(\vkfrom,\cdot)$ (i.e. $\vkfrom$ is fresh).
             \item Check that $\BS.\ver(\vk^\minter,\vkfrom,\sigma_\minter)=1$.
             \item Check that $\BS.\ver(\vkfrom,(\vkfrom,\vkto)=1$ (i.e. the sender certifies knowledge of the signing key relative to $\vkfrom$).
  %  \item Find $i$ such that $\assetvar[i]=(\vkfrom,\bot)$. If not found, abort the update.
    \end{itemize}
    If all the checks pass, Set $\assetvar[\genassets+1]=(\vkfrom,\vkto,0)$ and send $(\UPDATED,\vkfrom,\vkto)$ to $\party$.
%\item[Asset verification:] Upon receiving $(\VERIFY,\vkfrom,\vkto,\sigmato)$ from a party $\party\in\minters\cup\users$  does as follows:
%\begin{itemize}
    %\item Check that $\BS.\ver(\vk_T,\vk,\sigma_T)=1$ for at least a minter $\minter\in\minters$.
 %   \item Check that $\assetvar[i]=(\vkfrom,\vkto,\cdot)$ for at least an $i\in
 %   [\genassets]$. %(i.e. the asset $(\vkfrom,\vkto)$ exists and it is unspent).
%    \item Check that $\BS.\ver(\vkto,(\vkfrom,\vkto),\sigmato)=1$ (i.e., $\vkto$ is the recipient of the asset).
%\end{itemize}

%If all the checks above pass, return $(\VERIFIED,i,\vkfrom,\vkto,\sigmato)$ to $\party$, return $(\NOTVERIFIED,\vkfrom,\vkto,\sigmato)$ to $\party$ otherwise.

\item[Asset consume:] Upon receiving $(\SPEND,\vkfrom,\vkto,\sigmato)$ from a minter $\minter\in\minters$:
\begin{itemize}
    \item Check that $(\vkfrom,\vkto,0)$ is the last occurrence of $(\vkfrom,\vkto)$ in $\assetvar$ (i.e., the asset is not updated to spent).
    \item Check that $\BS.\ver(\vkto,(\vkfrom,\vkto),\sigmato)=1$ (i.e., $\vkto$ is the recipient of the asset).
\end{itemize}
If the checks above pass set $\assetvar[\genassets]=(\vkfrom,\vkto,1)$, and send $(\SPENT,\vkfrom,\vkto,\sigmato)$ to $\minter$, and send $(\NOTSPENT,\vkfrom,\vkto,\sigmato)$ otherwise.
\item[Asset information retrieaval:] On input $(\RETRIEVE)$ from any party $\party$, send $(\RETRIEVED,f_\aux(\assetvar))$ to $\party$.
\end{description}
    
\end{framed}

%From now on, we assume that parties periodically poll for the last DLT update by quering $\FuncBC$ with $(\readcom)$ to obtain $\chain$, and scanning $\chain$ anytime he wants to obtain some specific value.
%Let us say that each sender $\sender\in\users$ is connected with his own relay $\relay_\sender\in\relays$ and each bank $\bank$ is connected with her own  minter $\minter_\bank\in\minters$. 

The protocol is divided into the following phases:
\begin{description}
%\item[Setup:] During setup, the central bank $\cbank$ does the following:
%\begin{itemize}
   % \item Generates a blind signature pair of keys $(\BS.\vk_{\cbank},\BS.\sk_{\cbank})\getsr\BS.\Gen(1^\secpar)$ and distributes the central bank's verification key $\vk_{\cbank}$ to all the parties involved in the system along with a certificate. Certificate distribution and verification are outside our scope. 
%\end{itemize}
\item[Asset distribution:] 
Let us say that each bank $\bank$ in $\banks$ exchanged fiat money to receive a certain amount of assets $\genassets$ from the central bank (we assume that they all requested the same amount for the aim of simplicity).
The central bank $\cbank$ proceeds as follows:
\begin{itemize}
    \item Computes a verification key $\vk^{\cbank}$ and distributes it to all the parties $\parties$.
    \item Wait to receive $\tau$ verification keys from each bank (i.e. $\tau$ genesis assets from each bank).
    \item Wait to receive a key $\vk_\minter$ from each minter $\minter\in\minters$.
    \item  Instantiates $\FuncVer$ with the users $\users$, the banks $\banks$, minters $\minters$, minters verification keys $\{\vk^\minter\}_{\minter\in\minters}$, a variable
    $\assetvar$ containing $\genassets=|\banks|\cdot \tau$ genesis assets of the form $(\vk^{\cbank},\vk_i)$.
\end{itemize}

    \item[Asset withdrawal:] 
    We assume that each bank defined function $\checkreg(\cdot)$ for checking regulation compliance.
    The sender $\sender\in\users$ communicate with its bank $\bank\in\banks$, that will check whether $\sender$ has sufficient funds to obtain a new assets. 
    If so, the following steps are performed:
    \begin{itemize}
        \item $\sender$ computes $(\vk^\sender,\sk^\sender)\getsr\BS.\Gen(1^\secpar)$ and $\blinded^\sender=\blind(\vk^S,\bfactor^\sender)$ for a randomly generated $\bfactor\getsr\bin^\secpar$, and send $\blinded^\sender$ to $\bank$.
        \item $\bank$, owning a set of genesis assets of the type $\{(\vk^{\cbank},\vk^\bank)\}$,
      generates a signature $\sigma^\bank\getsr\BS.\sign(\sk^\bank,\allowbreak(\vk^{\cbank},\vk^\bank))$ for a randomly picked $\{(\vk^{\cbank},\vk^\bank)\}$, and forwards $(\vk^{\cbank},\vk^\bank,\sigma^\bank)$ together with the blinded message $\blinded^\sender$ received by $\sender$ to his own minter $\minter_\bank\in\minters$.
        \item $\minter_\bank$ queries $\FuncVer$ with $(\SPEND,\vk^{\cbank},\vk^\bank,\sigma^\bank)$.
        If receives $(\SPENT,\vk^{\cbank},\vk^\bank,\sigma^\bank)$ back from $\FuncVer$,
        generates $\bsigma^{\minter_\bank}\getsr\BS.\bsign(\sk^{\minter_\bank},\blinded^\sender)$ and forwards $\bsigma^{\minter_\bank}$ to $\bank$, that, in turn, forwards $\bsigma^{\minter_\bank}$ to $\sender$.
        \item $\sender$ can now obtain his own asset $\sigma^{\minter_\bank}=\unblind(\bsigma^{\minter_\bank},\bfactor^\sender)$. %and queries $\FuncVer$ with $(\CREATE,\vk^{\sender},\sigma^{\minter_\bank})$.
    \end{itemize}
 \item[Asset transfer:] Let us say that a receiver $\receiver$ has to receive an asset from a sender $\sender$. $\sender$ and $\receiver$ interact as follows:
 \begin{itemize}
    \item $\receiver$ computes $(\vk^\receiver,\sk^\receiver)\getsr\BS.\Gen(1^\secpar)$ and sends it to $\sender$.
     \item $\sender$, owning an asset $(\vk^\sender,\sigma^{\minter_\bank})$ where $\BS.\ver(\vk^{\minter_\bank},\vk^\sender,\sigma^{\minter_\bank})=1$,
     generates a signature $\sigma^\sender\getsr\sign(\allowbreak\sk^\sender,\allowbreak(\vk^\sender,\vk^\receiver,\sigma^{\minter_\bank}))$, and sends $(\vk^\sender,\sigma^\sender)$ to $\receiver$.
     \item $\receiver$ generates a signature $\sigma^\receiver\getsr\BS.\sign(\sk^\receiver,(\vk^\sender,\vk^\receiver,\sigma^{\minter_\bank}))$ and sends $(\vk^\sender,\vk^\receiver,\sigma^{\minter_\bank},\sigma^\receiver)$ to his own bank $\bank'$. 
     \item $\bank'$ queries $\FuncVer$ with $(\RETRIEVE)$ and receives back $(\RETRIEVED,\aux)$. If $\checkreg(\vk^\sender,\allowbreak\vk^\receiver,\sigma^\sender,\minter_\bank,\sigma^{\minter_\bank},\aux)=0$ (i.e., the asset is not regulation compliant), $\bank'$ withdraws the asset registration into the system, and aborts the execution.
     \item $\bank'$ queries $\FuncVer$ with $(\UPDATE,\vk^\sender,\allowbreak\vk^\receiver,\sigma^\sender,\minter_\bank,\sigma^{\minter_\bank})$. 
     \item The bank $\bank'$, if receiving $(\UPDATED,\vk^\sender,\vk^\receiver)$ from $\FuncVer$, forwards $(\UPDATED,\vk^\sender,\vk^\receiver)$ to $\receiver$, who can safely proceed with the exchange with the sender.
    
 \end{itemize}
  \item[Asset recycling:] $\sender$, owning a signing key $\sk'$ for an asset $(\vk,\vk')$, and its bank $\bank$, interact as follows:
  \begin{itemize}
      \item $\sender$ computes $\sigma'\getsr\BS.\sign(\sk',(\vk,\vk'))$,
      generates a new asset $\vk^\sender\getsr\BS.\Gen(1^\secpar)$ and sends $\blinded^\sender=\blind(\vk^\sender,\bfactor^\sender)$ to $\bank$, who forwards 
      $\blinded^\sender$ to her own minter $\minter_{\bank}$.
        \item $\minter_{\bank}$ queries $(\SPEND,\vk,\vk',\sigma')$. If it receives $(\SPENT,\vk,\vk',\sigma')$ from $\FuncVer$, computes $\bsigma^{T_{\bank}}\getsr\allowbreak\bsign(\vk^{\minter_{\bank}},\blinded^\sender)$ and sends it back to $\bank$, who forwards it to $\receiver$.
    \item $\receiver$ unblinds the asset $\sigma^{\minter_{\bank}}=\unblind(\bsigma^{\minter_{\bank}},\blinded^\receiver)$.%, and queries $\FuncVer$ with $(\CREATE,\vk^{\sender},\sigma^{\minter_\bank})$.
  \end{itemize}
  
 
  
\end{description}


==> pkifunc.tex <==

\begin{figure}
\begin{framed}
   The central bank $\cbank$ takes as an input a value $\tau$ indicating the number of assets that each bank $\bank\in\banks$ should receive and hold. First, Initializes a set of minters' keys $\mintkeys\gets\emptyset$. Then, setup is divided in the following phases:
    \begin{description}
               \item[Minter key collection:] Upon receiving $\vk^\minter$ from a minter $\minter\in\minters$  set $\mintkeys\gets\mintkeys\cup\{\vk^\minter\}$ (ignore any repeated query from the same minter).
               \item[Setup completion:] If $|\mintkeys|=|\minters|$:
               \begin{itemize}
                  \item Compute $(\vkcb,\skcb)\getsr\BS.\Gen(1^\secpar)$ and send $\vkcb$ to each $\party\in\parties$.
        \item Compute $\crs\getsr\nizk.\setup(1^\secpar)$.
        \item  For each $i\in[\tau]$ and each $\bank\in\banks$, compute $(\vk_i^\bank,\sk_i^\bank)\getsr\BS.\Gen(1^\secpar)$, where $F_1^{(\cbank,\bank)}$.
 
        \item Compute $\cbsigma\getsr\BS.\sign(\skcb,(\crs,\mintkeys,\{(\vkcb,\vk_i^\bank)\}_{i\in[\tau]),\bank\in\banks})$.
        \item Query $\FuncSC$ with $(\SET,\crs,\mintkeys,\{(\vkcb,\vk_i^\bank)\}_{i\in[\tau],\bank\in\banks},\crs,\cbsigma)$ and send $\{(\vk_i^\bank,\sk_i^\bank)\}_{i\in[\tau]}$ to each $\bank\in\banks$.
               \end{itemize}
    \end{description}

\end{framed}
    \caption{Central Bank Setup Phase}
    \label{fig:funccb}
\end{figure}


==> prel/vcom.tex <==
\subsection{Vector Commitments}
\begin{definition}[Vector Commitments]
Let $\msgspace$ be the message space.
    A vector commitment scheme $\VC$ is a tuple of algorithms $(\VC.\setup,\VC.\commit,\allowbreak\VC.\open,\VC.\ver)$ described as follows
    \begin{description}
        \item[$\VC.\setup(1^\secpar)$:] Outputs the public parameters $\pp$.
        \item[$\VC.\commit(\pp,\msg_1,\ldots,\msg_n)$:] Outputs a pair $(\com,\aux)$ where $\com$ is a commitment on the messages $\msg_i\in\msgspace$ for $i\in[n]$ together with some auxiliary information $\aux$.
        \item[$\VC.\open(\pp,\msg,i,\aux)$:] Outputs an opening proof $\opn$ for the $i$-th entry of the commitment.
        \item[$\VC.\ver(\pp,\com,\msg,i,\opn)$:] Outputs 1 if the opening proof $\opn$ verifies on index $i$ and message $\msg$ for the commitment $\com$, 0 otherwise.
    \end{description}
\end{definition}
We require the following properties
\begin{definition}[Perfect correctness]
    A vector commitment scheme $\VC$ satisfy {\em perfect correctness} if, for any $\msg_i\in\msgspace$ and for any index $i\in[n]$, it holds that
    \[\prob{\VC.\ver(\pp,\com,\msg,i,\opn)=1
    \Bigg |
\begin{tabular}{c}
     $\pp\getsr\setup(1^\secpar)$,  \\
$(\com,\aux)\getsr\VC.\commit(\pp,\msg_1,\ldots,\msg_n)$ \\
$\opn\getsr\VC.\open(\pp,\msg,i,\aux)$
\end{tabular}    
    }=1.\]
\end{definition}
\begin{definition}[Position binding]
    A vector commitment scheme $\VC$ satisfies computational positional binding if for any PPT adversary $\adv$, there exists a negligible function $\negl$ such that 
    \[\prob{
    \begin{tabular}{c}
$\VC.\ver(\pp,\com,\msg,i,\opn)=1$ \\
$\VC.\ver(\pp,\com,\msg',i,\opn')=1$ \\
$\msg\ne\msg'$
\end{tabular}
\Bigg |
    \begin{tabular}{c}
$\pp\getsr\setup(1^\secpar)$ \\
$(\com,\msg,\msg',i,\opn,\opn')\getsr\adv(\pp)$
\end{tabular}
}=1 \]
\end{definition}
\begin{definition}[$\epsilon$-succintntess]
    A vector commitment scheme is $\epsilon$-{\em succint} if there is a fixed $\epsilon(\secpar)$ such that, for any $n$, the size of the honestly generated commitment and openings is bounded by $\epsilon(\secpar)$.
\end{definition}
In our construction, we will consider  $(\poly\cdot \log n)$-succint vector commitment schemes.

==> prot-second-version.tex <==
section{Protocol Version 2}
We have the following actors
\begin{itemize}
    \item Minters for minting coins
    \item Users
    \item Banks
    \item Ledger
    \item Regulator revoking assets minted by malicious minters.
\end{itemize}
Possible idea: Allowing for a maximum number of mintable coins for each minter. If more coins than how much is supposed to are minted, payment traces starting from the malicious minter's coin are revoked.

About usage of ZKP: a user can show that his coin was minter correctly (i.e. from a burnt asset), but not that it is valid (the burnt asset could come from an invalid asset).

ZKP to identify trace of payment started from minter M 


==> techoverview.tex <==
In terms of security properties, our protocol shall guarantee the following properties:
\begin{description}
\item[Token anonymity:]  Banks are trusted in the sense that they will not disclose information about their users. The transaction between sender and receiver is marked with a nonce $\nonce$, who identifies the transaction the sender and the receiver agreed upon offline.
After a token is transferred, the sender/receiver cannot use the response of the functionality as a certificate do deanonymize the receiver/sender, since the random nonce is the only information disclosed to both.

\item[Token unforgeability and balance invariance:] During the setup phase, tokens can assigned only by the central bank $\cbank$. Then, token transfer, after checking that the sender had enough tokens in its wallet $\tokenvar_\sender$, moves a token from the sender's wallet to the receiver's wallet.
\end{description}
